Proof-of-Authorship for Diffusion-based AI Generated Content

Recent advancements in AI-generated content (AIGC) have introduced new challenges in intellectual property protection and the authentication of generated objects. We focus on scenarios in which an author seeks to assert authorship of an object generated using latent diffusion models (LDMs), in the presence of adversaries who attempt to falsely claim authorship of objects they did not create. While proof-of-ownership has been studied in the context of multimedia content through techniques such as time-stamping and watermarking, these approaches face notable limitations. In contrast to traditional content creation sources (e.g., cameras), the LDM generation process offers greater control to the author. Specifically, the random seed used during generation can be deliberately chosen. By binding the seed to the author's identity using cryptographic functions, the author can assert to be the creator of the object. We refer to this stronger guarantee as proof-of-authorship, since only the creator of the object can legitimately claim the object. This contrasts with proof-of-ownership via time-stamping or watermarking, where any entity could potentially claim ownership of an object by being the first to timestamp or embed the watermark. We propose a proof-of-authorship framework involving a probabilistic adjudicator who quantifies the probability that a claim is false. Furthermore, unlike prior approaches, the proposed framework does not involve any secret. We explore various attack scenarios and analyze design choices using Stable Diffusion 2.1 and XL as representative case studies.

==> tables/perceptual_hash.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\caption{For related images, the results are computed by comparing a LDM generated base image with its transformed variants, and for unrelated images, we compare pairs of randomly generated LDM images. Mean Diff. refers to the difference between the means computed over related and unrelated images. PDQ (in bold) is employed as it has the largest mean difference.}

\label{table:perceptual_hash_eval}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|cc|cc|c|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Perceptual\\ Hash\end{tabular}} & \multicolumn{2}{c|}{Unrelated} & \multicolumn{2}{c|}{Related}  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Mean\\ Diff.\end{tabular}} \\ \cline{2-5}
                                                                           & Mean           & Std. Dev      & Mean          & Std. Dev      &                                                                       \\ \hline
\textbf{PDQ}                                                               & \textbf{0.45}  & \textbf{0.05} & \textbf{0.13} & \textbf{0.15} & \textbf{0.32}                                                         \\
pHash                                                                      & 0.42           & 0.06          & 0.12          & 0.16          & 0.3                                                                   \\
wHash                                                                      & 0.36           & 0.1           & 0.09          & 0.13          & 0.27                                                                  \\ \hline
\end{tabular}%
}
\end{table}

==> tables/poa_prob_table.tex <==
\begin{table*}[]
\centering
\caption{The probabilities computed using the latent space and feature similarity metrics, together with the overall probablity that is returned by the probabilitistic adjudicator. Categories 1, 2 and 3 refer to the categories of images described in Section \ref{section:poa_evaluation}. }
\label{table:poa_probability}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{Category} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Latent Space\\ Similarity\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Feature\\ Similarity\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Overall\\ Probability\end{tabular}} \\ \cline{2-10} 
                          & Min                        & Mean                      & Std. Dev                      & Min                      & Mean                     & Std. Dev                    & Min                      & Mean                     & Std. Dev                     \\ \hline
1                         & 0.93                       & 0.97                      & 0.01                          & 1.00                     & 1.00                     & 0.00                        & 0.93                     & 1.00                     & 0.00                         \\
2                         & 0                          & 0.14                      & 0.02                          & 0.78                     & 0.83                     & 0.02                        & 0.78                     & 0.83                     & 0.01                         \\
3                         & 0.00                       & 0.00                      & 0.00                          & 0.38                     & 0.47                     & 0.04                        & 0.38                     & 0.47                     & 0.06                         \\ \hline
\end{tabular}%
% }
\end{table*}
